Exploiting Defenses against GAN-Based Feature Inference Attacks in Federated Learning

Federated learning (FL) is a decentralized model training framework that aims to merge isolated data islands while maintaining data privacy. However, recent studies have revealed that Generative Adversarial Network (GAN) based attacks can be employed in FL to learn the distribution of private datasets and reconstruct recognizable images. In this paper, we exploit defenses against GAN-based attacks in FL and propose a framework, Anti-GAN, to prevent attackers from learning the real distribution of the victim's data. The core idea of Anti-GAN is to manipulate the visual features of private training images to make them indistinguishable to human eyes even restored by attackers. Specifically, Anti-GAN projects the private dataset onto a GAN's generator and combines the generated fake images with the actual images to create the training dataset, which is then used for federated model training. The experimental results demonstrate that Anti-GAN is effective in preventing attackers from learning the distribution of private images while causing minimal harm to the accuracy of the federated model.

==> tex/responseletter-v1.tex <==
\onecolumn

\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{10mm}

% \begin{auxmulticols}{2}

We would like to thank all the reviewers for their insightful and constructive comments. We have carefully addressed the comments and have highlighted the major changes in the revised paper in {\color{blue} blue}.

\section*{Summary of Changes}
\label{sec-changes}

% \begin{itemize}
    % \item 
%We have repeated the experiments relevant to Random Forest, changing the number of trees from 20 to 100, and implemented two new experiments for testing the impact of increasing query size with two real-world datasets. We added explanations and discussions on the questions raised in the review, and gave examples for each of the proposed methods.
% \end{itemize}

\begin{itemize}[topsep=2pt,itemsep=2pt,parsep=0pt,partopsep=0pt,leftmargin=10pt]
    \item In Section~\ref{sec-intro}, we have revised the discussion on the limitations of DP-based and crypto-based defense methods and clarified the focus of our attack target.
    \item  In Section~\ref{subsec-mixup}, we have provided additional justification for the use of two-image mixing in \scheme, along with the inclusion of  Algorithm~\ref{alg-framework-antigan} to illustrate the overview of the proposed \scheme framework.
    \item  In Section~\ref{subsec-exp-comp-dp}, we have added experimental results on the CIFAR10 dataset, and results on a new baseline method, the Dropout-based method~\cite{scheliga2023dropout}. 
    \item  We have added a new section, Section~\ref{subsec-evaluate-visual-features}, to evaluate the privacy leakage of \scheme across different visual features.
    \item  We have added a new section, Section~\ref{sec-exp-client}, to evaluate the performance of \scheme under different client configurations.
    \item In Section~\ref{apdx-exp-ablation}, we have added a new ablation experiment to evaluate the effectiveness of the choice on the feature extractor.
    \item we have expanded the discussions on related work previously in Section 2.3 and 6 into a new section, Section~\ref{sec-related-work}, for a more comprehensive review of related studies.
    \item We have expanded the conclusion section, Section~\ref{sec-conclusion}, to reflect the quantitative values and metrics in our experiments.
\end{itemize}





% \section*{Response to Meta-Reviewer}
% \noindent
% \textbf{Comment 1.} The reviewers liked the paper and would like to see a revision. Each reviewer lists a reasonably concrete list of suggestions. Please try to address them all.

% \vspace{2mm}\noindent
% \textbf{Response.} We have carefully addressed the comments point by point and revised the paper.

\section*{Response to Reviewer 1}
\noindent
\textbf{W1.} Why is the first layer of ResNet chosen to extract classification features instead of utilizing other classification models like DenseNet? Could you add an experiment to substantiate this choice?

\vspace{2mm}\noindent
\textbf{Response.} We have added an ablation study in Section~\ref{apdx-exp-ablation} to evaluate the impact of different choices of $C$ on the defense performance of \schemens.
%
In this experiment, we replace the first convolutional layer of ResNet-18 with that of a pre-trained DesNet-121~\cite{densenet} as the feature extractor $C$. The results have been included in Table~\ref{tab-ablation}, from which we can see that the defense performance of \scheme on the DenseNet feature extractor is comparable to the performance on the ResNet extractor, indicating that the first convolutional layers of various pre-trained deep models can be effectively utilized within the \scheme framework.
%
The related discussions have been included in Section~\ref{apdx-exp-ablation}.

\vspace{2mm}\noindent
\textbf{W2.} Why does the Mixup process involve only mixing 2 images rather than 3 or more?

\vspace{2mm}\noindent
\textbf{Response.} Because mixing three or more images could lead to model performance degradation and increased computational costs during model training. The issue has been discussed in \cite{zhang2017mixup} and empirically validated in \cite{huang2020instahide}. We have provided more discussion in Section~\ref{subsec-mixup} to address this concern.


\section*{Response to Reviewer 2}
\noindent
\textbf{W1.} There is another popular method called InstaHide which has similar spirit to Anti-GAN, i.e., obfuscating the visual features of training images. However, the authors fail to compare the proposed method with InstaHide. I suggest that the authors provide more explanations on the difference between Anti-GAN and Instahide, specifically, what are the pros and cons when comparing Anti-GAN with InstaHide.

\vspace{2mm}\noindent
\textbf{Response.} As suggested, we have added more discussions on the similarities and differences between \scheme and InstaHide in Section~\ref{sec-related-work}. Generally, InstaHide~\cite{huang2020instahide} is similar in spirit to our approach, i.e., using \emph{Mixup}~\cite{zhang2017mixup} to corrupt the visual features of private training images. However, there are three main differences between \scheme and InstaHide.
%
First, InstaHide mixes multiple real images into one training image, while our scheme uses a GAN model to generate multiple fake images and then mixes these fake images with real images.
%
Second, InstaHide obfuscates image visual features by randomly flipping pixel signs, leading to uncontrollable model performance degradation. In contrast, \scheme obfuscates visual features using a specifically designed loss function, allowing the privacy-utility tradeoff to be tuned for different application scenarios.
%
Third, \cite{carlini2020attack} and \cite{luo2021fusion} have experimentally demonstrated that private images can be reconstructed from the mixup images generated by InstaHide on the condition that the same private image is mixed into multiple training images. Our scheme mitigates this risk by ensuring that each private image is mixed only once.



\vspace{2mm}\noindent
\textbf{W2.} In addition, the target defense effect is unclear. From figure 5 and figure 7, I can see that although Anti-GAN eliminates the details inferred by GAN-based attacks and gradient inversion attacks, the outlines of objects and human faces are still distinguishable. If the authors aim to damage the details instead of outlines, they should explicitly justify the target defense effect in the beginning of this paper.


\vspace{2mm}\noindent
\textbf{Response.} We have added more discussions in Section~\ref{sec-intro} to justify the target defense effect. Specifically, \scheme is designed to obfuscate object details rather than the entire visual features of training images. \scheme can preserve the semantic information necessary for the downstream classifier, such as the outline of a human face, while rendering object details, such as eyes and noses, indistinguishable to the human eye. Consequently, our scheme can significantly reduce the accuracy degradation caused to the federated model and ensure that images reconstructed by attackers are rendered useless.

\vspace{2mm}\noindent
\textbf{W3.} For the experiments, I would like to see the defense effects of Anti-GAN on other complicated datasets, e.g., CIFAR10. I suggest the authors provide experiments on CIFAR10 to validate the generalization of the proposed method.

\vspace{2mm}\noindent
\textbf{Response.} As suggested, we have conducted additional experiments on CIFAR10 using \schemens, the DP-based FL framework~\cite{shokri2015privacy}, and the Dropout-based method~\cite{scheliga2023dropout}. The corresponding results have been included in Table~\ref{tb-comp}. These results demonstrate that the accuracy degradation rates and reconstruction similarity scores for \scheme on CIFAR10 follow a pattern consistent with those observed on MNIST, FashionMNIST, and CelebA, validating the generalization of the proposed method.
%
We have revised the discussions in Section~\ref{subsec-exp-comp-dp} accordingly to reflect the new CIFAR10 results.







\section*{Response to Reviewer 3}
\noindent
\textbf{W1.} More GAN-based inference attacks should be considered in the experiments.


\vspace{2mm}\noindent
\textbf{Response.} In Section~\ref{sec-problem}, we discussed two different GAN-based attacks: client-side attack~\cite{hitaj2017deep} and server-side attack~\cite{wang2019beyond}. Given the similarity in attack techniques employed by these two types of attacks, the resulting attack outcomes in our experiments are also similar across different settings. Therefore, for clarity, we presented only the attack results generated by \cite{hitaj2017deep} in our experiments. We have added more explanations in Section~\ref{subsec-exp-setting} to highlight the similarity in attack results between \cite{hitaj2017deep} and \cite{wang2019beyond}.



\vspace{2mm}\noindent
\textbf{W2.} Only DP-based defence is considered, please add more methods as comparisons.

\vspace{2mm}\noindent
\textbf{Response.} Aside from DP-based defense methods, we have also added new experiments to compare \scheme with a Dropout-based defense method~\cite{scheliga2023dropout}, which was designed to counteract gradient-matching attacks~\cite{zhu2020deep} by regularizing the model to prevent it from memorizing private training data.  
%
For the Dropout-based method, we followed the parameter setting in \cite{scheliga2023dropout} and set the dropout rates $p\in \{0.1, 0.5\}$ after each layer of the testing models.
%
The ADRs and SSIMs obtained from the Dropout-based method~\cite{scheliga2023dropout} are included in Table~\ref{tb-comp}.
%
The main observation is that the Dropout-based method~\cite{scheliga2023dropout} incurs minimal accuracy degradation compared to \scheme and, under certain conditions, even enhances model performance. This is anticipated as the method in \cite{scheliga2023dropout} can act as a regularization approach that can improve the model's generalization performance. However, its defensive efficacy, as reflected in the SSIM scores for image reconstruction, is the lowest among the three methods. This suggests that the Dropout-based method is less effective in preventing the memorization of training image distributions, thereby offering limited protection against GAN-based attacks~\cite{hitaj2017deep}.
%
We have added the related discussions in Section~\ref{subsec-exp-setting} and \ref{subsec-exp-comp-dp}.




\vspace{2mm}\noindent
\textbf{W3.} The related work should be improved, As I know, some GAN-based attacks are used for backdoor attacks, like bellow:
[1] H. Mei, G. Li, J. Wu and L. Zheng, "Privacy Inference-Empowered Stealthy Backdoor Attack on Federated Learning under Non-IID Scenarios," 2023 International Joint Conference on Neural Networks (IJCNN), Gold Coast, Australia, 2023, pp. 1-10.

\vspace{2mm}\noindent
\textbf{Response.} As suggested, we have expanded the discussions on related work previously in Section 2.3 and 6 into a new section, Section~\ref{sec-related-work}, to include other types of GAN-based attacks, including the one highlighted by the reviewer.  
%
Note that in the literature, GANs have also been used in other types of attacks, such as membership inference attacks~\cite{chen2020gan-membership,lin2021gan-membership-privacy}, backdoor attacks~\cite{mei2023gan-backdoor-privacy,hu2022gan-backdoor-generating}, and adversarial attacks~\cite{zhu2023gan-adversarial-frequency,na2022gan-adversarial-unrestricted}. However, this paper specifically focuses on \textit{GAN-based feature inference attacks}.



\section*{Response to Reviewer 4}
\noindent
\textbf{W1.} The privacy risk is only measured as the reconstruction similarity. The low level features are kept through the feature extractor C, such that the FL model can learn the features related to object detection. However, it is unclear if any privacy features are also kept. There should be another evaluation on the attacker side. Even if the reconstructed image quality is low, can the attackers use these low quality image to perform inference on privacy information (e.g., gender, age, identity, etc.).


\vspace{2mm}\noindent
\textbf{Response.} We have added new experiments on the CelebA dataset to evaluate whether an attacker can exploit low-quality images generated by \scheme to infer various private visual features. Specifically, we investigate whether \schemens, trained on the gender classification task, can protect the privacy of additional visual features such as hair color and eyeglasses. 
%
In the experiment, we first train classifiers on real images labeled with various visual attributes including black hair, eyeglasses, smiling, and young. 
%
These classifiers, once well-trained, are then utilized to predict the labels of images generated by \schemens. We employ entropy to quantify the uncertainty of model predictions post-softmax~\cite{van2020uncertainty}: $H(p)=-\sum_i p_i(x)\log p_i(x)$, where $p_i(x)$ denotes the probability of $x$ being assigned label $i$ in the model predictions, and higher $H(p)$ values indicate greater uncertainty in the model's predictions. 
%
The entropy values of model predictions on \scheme for the visual features $\{\text{black hair}, \text{eyeglasses}, \text{smiling}, \text{young}\}$ are $\{0.5846,	0.5574,	0.6086,	0.631\}$, respectively. 
%
For comparison, the entropy values of model predictions on real images for the four visual features are $\{0.4167,	0.1929,	0.3426,	0.5211
\}$, and the entropy of random guesses is 0.6931.
%
These results demonstrate that \scheme can substantially increase the uncertainty in model predictions on the generated images with obfuscated visual features, nearly to the level of random guesses, thus significantly mitigating the risks of privacy leakage for various visual features.
%
The new experimental results and related discussions have been included in Section~\ref{subsec-evaluate-visual-features}.





\vspace{2mm}\noindent
\textbf{W2.} “the memorization nature of ML models [8]”  only deep NN models, not traditional ML models.

\vspace{2mm}\noindent
\textbf{Response.} We have revised this phrase to "the memorization nature of neural network models".

\vspace{2mm}
\noindent
\textbf{W3.} Figure 4 caption is wrong.

\vspace{2mm}\noindent
\textbf{Response.} We have revised the caption of Figure~\ref{fig-parameter-comparison} to "(a)-(b): the accuracy degradation of the federated model and the performance of GAN-based attacks under \scheme with different pixel variances $v_e$ and $\mu=0.5$; (c)-(d): the accuracy degradation and attack performance tested under \scheme with different mixup parameters $\mu$ and $v_e=0.5$" to eliminate possible misunderstandings.






\section*{Response to Reviewer 5}
\noindent
\textbf{W1.} I recommend revising the first 3 paragraphs of the Introduction section by considering two aspects: (1) In some places, the paper states that Anti-GAN’s property is stopping “group-level” attacks and group reconstruction, rather than record-level reconstruction. However, much of the experimental evaluation is done on individual samples (record-level), not group-level. Anti-GAN method is also inherently record-level. Thus, this argument seems contradictory to the paper’s content. (2) The criticisms against existing defenses (e.g., DP-based and crypto-based) are not fair. In particular, according to the threat model of the paper, if encryption was used then the attacker would not be able to see the gradients in plaintext and would not be able to run the attack. Similarly, DP-based defenses are also somewhat effective against the studied attacks (as expected, and as the experiments show).


\vspace{2mm}\noindent
\textbf{Response.} (1) We would like to note that the two evaluation metrics in our experiments, accuracy degradation ratio and SSIM scores, are based on group-level data. Specifically, the accuracy degradation ratio is evaluated on the entire generated dataset, while SSIM scores assess the similarity between two groups of images (see Eq.~\ref{eq-ssim-exp} for more details). 
%
We also note that in Fig.~\ref{fig-two-eggs}, the images $\Tilde{x}$ generated by GAN-based attacks do not correspond to $\hat{x}$ produced by \scheme in a one-to-one manner, as GAN models are capable of generating only class representations rather than the original training images. We have added additional explanations in the caption of Fig.~\ref{fig-two-eggs} to clarify the correspondence between $\Tilde{x}$ and $\hat{x}$. 
%
In addition, our experimental results in Section~\ref{sec-defend-gradient-matching} have demonstrated that, beyond countering group-level attacks, \scheme can effectively mitigate record-level attacks. We have added further discussions in Section~\ref{sec-intro} to highlight the effectiveness of \scheme against record-level attacks. Nevertheless, we would like to emphasize that \scheme is initially designed to defend against group-level attacks.
%
(2) Regarding the crypto-based defenses, we acknowledge their potential in defending the attack scenario in \cite{hitaj2017deep}, but they have limitations in the FL context. Specifically, traditional cryptographic methods, such as homomorphic encryption~\cite{wu2020privacy, keller2020mp} and secure multiparty computation~\cite{bonawitz2017practical, Mohassel17}, require significant computational resources~\cite{wu2020privacy,zhang2020batchcrypt,truex2019hybrid}, thereby restricting their application scenarios. In addition, encrypting local gradients can inhibit anomaly detection methods designed to counteract poisoning-based attacks~\cite{jiang2024distribution, bagdasaryan2018backdoor}. 
%
We have revised our claims in Section~\ref{sec-intro} accordingly. Regarding DP-based methods, we would like to note that they provide limited protection against group-level attacks, as they are primarily designed to prevent record-level privacy leakage~\cite{shokri2017membership} instead of protecting group-level information~\cite{jiang2024distribution}. We have highlighted these points in Section~\ref{sec-intro} for reference.




\vspace{2mm}\noindent
\textbf{W2.} In Section 3, it is stated that attacker A (acting as an FL participant) downloads the shared gradients of victim V and utilizes them to update the discriminator of the attack GAN model. However, in general, it is assumed that FL participants do not have direct access to other individual participants’ gradients. Instead, a participant receives the aggregated result after the FL server combines many victims’ gradients. Hence, this paper’s assumption that A receives V’s gradients seems to contradict the general setup of FL. Please clarify or provide references in which the paper’s assumption holds.

\vspace{2mm}\noindent
\textbf{Response.} This two-client attack scenario is used in the baseline attack \cite{hitaj2017deep}, and we follow it to design the corresponding defense method in this paper. In Section~\ref{sec-problem}, we have added more explanations to justify this attack scenario.
%
Specifically, unlike traditional FL scenarios~\cite{mcmahan2016communication}, where participants receive only aggregated global gradients, the two-client scenario used in \cite{hitaj2017deep} allows the attacker to directly receive the victim's gradients. This direct access poses substantial challenges for designing defense methods because, compared to traditional FL scenarios where gradient aggregation can balance out the private information contained in the victim's gradients~\cite{wei2020framework}, the two-client scenario directly exposes the possible private information to attackers. Correspondingly, if our method can effectively mitigate information leakage in the stringent two-client scenario, it can also be adopted in traditional FL scenarios, achieving equal or superior defense effects.




\vspace{2mm}
\noindent
\textbf{W3.} Section 4 would benefit from a general “defense overview” algorithm to show how the individual steps (explained in Sections 4.1 to 4.3) are put together.

\vspace{2mm}\noindent
\textbf{Response.} As suggested, we have summarized the main steps of Anti-GAN in Algorithm~\ref{alg-framework-antigan} to demonstrate the defense overview.




\vspace{2mm}
\noindent
\textbf{W4.} The experiments assume a two-client FL setup, which is overly simplistic in today’s FL settings. I would have expected experiments with varying numbers of clients and iid vs non-iid data distributions so that the effectiveness of the defense could be measured in more realistic settings. For example, how is Anti-GAN impacted when the number of data samples per class is low? How is it impacted when the data distribution is non-iid? Convergence of the victim-side GAN model can be challenging in such scenarios, limiting the applicability of Anti-GAN.

\vspace{2mm}\noindent
\textbf{Response.} We have added new experiments to evaluate the performance of \scheme under different client configurations within the FL framework. The numbers of clients are chosen from $\{ 2,4,8,26,32\}$. Note that GAN-based attacks~\cite{hitaj2017deep} are effective only in scenarios where the adversary does not possess the target data distribution, which means that the data distribution among different clients in FL should be heterogeneous, non-iid distributions.
%
In the experiment, we first randomly divide the training data into two halves based on class distribution and similarly partition the clients into two groups. Then, each client in the first group is assigned a specific number of data samples randomly chosen from the first half of the training set, while clients in the second group receive samples from the second half. This approach ensures that the data distributions between the two client groups differ significantly, thereby enabling the attacker in one group to infer the data distribution of a defender in the opposite group using GAN-based attacks. 
%
To more accurately reflect real-world FL scenarios, we progressively reduce the number of samples per client as the number of clients increases. Specifically, the sample sizes per client for client configurations $\{2, 4, 8, 26, 32\}$ are set to $\{6000, 4000, 2000, 1000, 500\}$, respectively.
%
Table~\ref{tb-comp-diff-clients} presents the performance of \scheme across different client configurations.
%
Notably, as the number of clients in the FL framework increases, the degradation in accuracy caused by \scheme diminishes. This trend is due to the reduction in data samples per client as the number of clients rises, which leads to fewer generated samples being used by the defender during training, thereby mitigating the negative impact of \scheme on the performance of the federated model.
%
Furthermore, the data in Table~\ref{tb-comp-diff-clients} demonstrate that as the number of clients increases, the defense performance of \scheme improves, reflected by a reduction in SSIM scores for image reconstruction. This improvement can be attributed to the limitations of GAN-based attacks~\cite{hitaj2017deep}, which depend on the gradients uploaded by the defender to train the adversarial generator. As the number of samples owned by the defender decreases, the useful information in the uploaded gradients diminishes, thereby hindering the adversary's ability to generate plausible images.
%
In summary, increasing the number of participating clients in the FL framework can enhance the performance of \schemens.
%
The new experimental results and related discussions are included in  Section~\ref{sec-exp-client}.

\vspace{2mm}
\noindent
\textbf{W5.} In Section 2.3 and Section 6, the paper would benefit from a more detailed and up-to-date discussion of related works. There have been numerous related works on defending against gradient leakage attacks and data reconstruction attacks in FL in recent years, which can be adapted to the paper’s scenario.

\vspace{2mm}\noindent
\textbf{Response.} As suggested, we have expanded the discussions on related work in Section 2.3 and Section 6 into a new section, Section~\ref{sec-related-work} Related Work. In this new section, we detailedly discuss the state-of-the-art studies on defending against data reconstruction attacks in FL. Specifically, we first discuss related studies on inference attacks on machine learning, including membership inference~\cite{shokri2017membership,salem2018ml,nasr2019comprehensive, melis2019exploiting}, property inference~\cite{propertyFL, propertyPermutation, propertyPoison, melis2019exploiting,jiang2024distribution}, and feature inference (also known as model inversion)~\cite{fredrikson2015model, luo2020feature, wu2016methodology, zhu2020deep,hitaj2017deep,wang2019beyond,luo2022feature,jayaraman2022attribute}. 
%
Subsequently, we discuss the corresponding defenses against these inference attacks, including dropout~\cite{melis2019exploiting,salem2018ml,scheliga2023dropout}, model stacking~\cite{salem2018ml}, mutual information-based regularization~\cite{wang2021improving}, anomaly detection~\cite{bagdasaryan2018backdoor}, differential privacy~\cite{shokri2015privacy,bagdasaryan2018backdoor,geyer2017differentially,jiang2024protecting,guo2022bounding}, secure multiparty computation~\cite{wu2020privacy, Mohassel17,bonawitz2017practical,zhang2020batchcrypt,truex2019hybrid}, and InstaHide~\cite{huang2020instahide}. In addition, we discuss the main differences between current defense methods and our approach in Section~\ref{sec-related-work}. We refer the reviewer to Section~\ref{sec-related-work} for more details.






\section*{Response to Reviewer 6}
\vspace{2mm}
\noindent
\textbf{W1.} There are too many references to non-peer-reviewed venues like arXiv. These references cannot be leveraged to support a claim or conduct a comparison as they are yet to be peer-reviewed.

\vspace{2mm}\noindent
\textbf{Response.} We acknowledge this issue and have made revisions to address it. Specifically, we have updated the publication venues for \cite{gulrajani2017improved,bagdasaryan2018backdoor,carlini2018secret,adam,mcmahan2016communication,radford2015unsupervised,salem2018ml,wu2020privacy,xiao2018generating,zhang2017mixup} from arXiv to their respective peer-reviewed conferences or journals. In addition, we have added new peer-reviewed references \cite{keller2020mp,shorten2019survey,zhang2022understanding,jiang2024protecting} to support our claims. The remaining arXiv references are \cite{mirza2014conditional, FashionMNIST, opacus}. Here, \cite{FashionMNIST} is a widely used dataset, \cite{opacus} refers to a PyTorch library, and \cite{mirza2014conditional} discusses Conditional GANs (over 13340 citations on Google Scholar).
%
We have ensured that these three arXiv references are not used to support a claim or for comparisons in our paper.






\vspace{2mm}
\noindent
\textbf{W2.} Conclusion section should be expanded and reflect the research outcome in terms of quantitative values and metrics.

\vspace{2mm}\noindent
\textbf{Response.} As suggested, we have expanded the conclusion section to reflect the quantitative values and metrics in our experiments. Specifically, in this paper, we introduce \scheme, a novel approach designed to protect the privacy of participants' training data against GAN-based feature inference attacks in the context of federated learning. By strategically distorting the original distribution of the private training dataset, \scheme effectively prevents attackers from generating distinguishable images while maintaining a high-performance federated classifier. 
%
Our experimental results demonstrate that, compared to the widely adopted DP-SGD mechanism, which can degrade model accuracy by up to $12\%$ and allow for a similarity score of up to 0.53 for image reconstruction, our method limits model accuracy degradation to a maximum of $5\%$ and reduces the similarity scores of reconstructed images to at most 0.30. In addition, our experiments show that \scheme can not only defend against GAN-based feature inference attacks but also provide protection against gradient-based record-level reconstruction attacks.
%
This study represents an initial step toward developing defense mechanisms against GAN-based attacks that can achieve a favorable privacy-utility tradeoff, and we believe it can contribute valuable insights into the advancement of privacy-preserving mechanisms in the context of federated learning.




\vspace{2mm}
\noindent
\textbf{W3.} The study of related work seems shallow. It should be expanded to cover all related studies.

\vspace{2mm}\noindent
\textbf{Response.} We have expanded the paragraph regarding related work into a new section, Section~\ref{sec-related-work} Related Work. In this section, we first discuss related studies on inference attacks on machine learning, including membership inference~\cite{shokri2017membership,salem2018ml,nasr2019comprehensive, melis2019exploiting}, property inference~\cite{propertyFL, propertyPermutation, propertyPoison, melis2019exploiting,jiang2024distribution}, and feature inference (also known as model inversion)~\cite{fredrikson2015model, luo2020feature, wu2016methodology, zhu2020deep,hitaj2017deep,wang2019beyond,luo2022feature,jayaraman2022attribute}. 
%
Subsequently, we discuss the corresponding defenses against these inference attacks, including dropout~\cite{melis2019exploiting,salem2018ml,scheliga2023dropout}, model stacking~\cite{salem2018ml}, mutual information-based regularization~\cite{wang2021improving}, anomaly detection~\cite{bagdasaryan2018backdoor}, differential privacy~\cite{shokri2015privacy,bagdasaryan2018backdoor,geyer2017differentially,jiang2024protecting,guo2022bounding}, secure multiparty computation~\cite{wu2020privacy, Mohassel17,bonawitz2017practical,zhang2020batchcrypt,truex2019hybrid}, and InstaHide~\cite{huang2020instahide}. In addition, we discuss the main differences between current defense methods and our approach in Section~\ref{sec-related-work}. We refer the reviewer to Section~\ref{sec-related-work} for more details.



\vspace{2mm}
\noindent
\textbf{W4.} Although DP-SGD has been considered state-of-the-art and a base for conducting experiments and comparing results, there is room for improving the comparison against more related works, in particular those that have employed MNIST, FashionMNI, and CelebA datasets.

\vspace{2mm}\noindent
\textbf{Response.} Aside from DP-based defense methods, we have also added new experiments to compare \scheme with a Dropout-based defense method~\cite{scheliga2023dropout}, which was designed to counteract gradient-matching attacks~\cite{zhu2020deep} by regularizing the model to prevent it from memorizing private training data.  
%
For the Dropout-based method, we followed the parameter setting in \cite{scheliga2023dropout} and set the dropout rates $p\in \{0.1, 0.5\}$ after each layer of the testing models.
%
The ADRs and SSIMs obtained from the Dropout-based method~\cite{scheliga2023dropout} are included in Table~\ref{tb-comp}.
%
The main observation is that the Dropout-based method~\cite{scheliga2023dropout} incurs minimal accuracy degradation compared to \scheme and, under certain conditions, even enhances model performance. This is anticipated as the method in \cite{scheliga2023dropout} can act as a regularization approach that can improve the model's generalization performance. However, its defensive efficacy, as reflected in the SSIM scores for image reconstruction, is the lowest among the three methods. This suggests that the Dropout-based method is less effective in preventing the memorization of training image distributions, thereby offering limited protection against GAN-based attacks~\cite{hitaj2017deep}.
%
We have added the related discussions in Section~\ref{subsec-exp-setting} and \ref{subsec-exp-comp-dp}.


% \end{auxmulticols}


==> tex/responseletter-v2.tex <==
\onecolumn

\centerline{\textbf{\Large Response to Reviewers' Comments (Minor Revision)}}
\vspace{10mm}

% \begin{auxmulticols}{2}

We thank all the reviewers for their additional feedback. We have carefully addressed the comments and have highlighted the major changes in this version in {\color{magenta} magenta}.
%
Changes in the previous version remain highlighted in
{\color{blue} blue}.



\section*{Response to Reviewer 1}
\noindent
\textbf{W1.} The newly added 5.5 Evaluation of Privacy Leakage on Different Visual Features only evaluate on uncertainty (in terms of entropy) of privacy inference attack without accuracy. They should be compared together to support the conclusion.


\vspace{2mm}\noindent
\textbf{Response.} We appreciate the reviewer’s suggestion that classification accuracy data can further support the conclusion. However, we would like to note that classification accuracies are not available in this experiment because \scheme generates images labeled exclusively for the primary gender classification task. As a result, ground-truth labels for other visual features are unavailable, making it impossible to compute classification accuracies for attributes beyond gender.
%
Instead, we choose to employ entropy to quantify the uncertainty of model predictions.
%
This discussion has been included in Section~\ref{subsec-evaluate-visual-features}.




\section*{Response to Reviewer 2}
\noindent


\vspace{2mm}\noindent
\textbf{Response.} We thank the reviewer for the positive feedback and for recommending the acceptance of our paper. We appreciate the recognition of our contributions and the insights for improving the manuscript. We are grateful for the support.







\section*{Response to Reviewer 3}
\noindent
\textbf{W1.} In the Introduction, it is stated that protecting group-level information is not guaranteed by the definition of DP. However, if an algorithm satisfies eps-DP, then it can be generalized to group-level by (k*eps)-DP for a group of size k. Thus, it is not clear why DP cannot protect group-level information. This part can be strengthened by providing a more concrete example or additional references with more detailed explanations.


\vspace{2mm}\noindent
\textbf{Response.} As suggested, we have strengthened this part by adding more references and discussions to justify this claim.
%
Specifically, DP is initially designed for protecting individual records, and protecting group-level information surpasses the initial scope of DP's privacy guarantee.  
%
For example, recent work~\cite{jiang2024distribution} has demonstrated the ability to extract training data distributions from FL systems protected by DP. 
%
While extensions of DP to group-level privacy have been explored~\cite{geyer2017differentially,jiang2024protecting}, these approaches often compromise model performance under moderate privacy budgets~\cite{geyer2017differentially}, and the application scenarios are typically limited to simple models like logistic regression or support vector machines~\cite{jiang2024protecting}.
%
These discussions have been included into the revised introduction.



\vspace{2mm}\noindent
\textbf{W2.} I recommend revising the Introduction section so that the newly added material is better integrated with the existing material. In the current state, some arguments seem to be repeated in multiple places, e.g., why is DP not sufficient, why are cryptographic approaches not sufficient. Making one pass over the whole Introduction section would address these issues.

\vspace{2mm}\noindent
\textbf{Response.} As suggested, we have revised the introduction section to eliminate redundancies and merge discussions on the limitations of DP and cryptographic approaches.
%
The revised introduction section is now more concise and fluent, meanwhile highlighting the motivation for our work.


\vspace{2mm}\noindent
\textbf{W3.} Section 5.6: The numbers in the text contain a typo that is repeated twice: 26 -> 16.

\vspace{2mm}\noindent
\textbf{Response.} We thank the reviewer for pointing out these two typos and have corrected them in this revision. We have also carefully checked all newly added content to ensure accuracy.




\vspace{2mm}\noindent
\textbf{W4.} The Related Work section was added, and it has strengthened the paper. However, the current Related Work section lists and discusses the related works without much grouping. Therefore, the precise positioning of the paper remains unclear. First, I suggest dividing the Related Work section into subsections and/or paragraphs by grouping relevant works together. Second, the main shortcomings and differences of Anti-GAN compared to groups of works or individual works when necessary (such as InstaHide) can be given.


\vspace{2mm}\noindent
\textbf{Response.} As suggested, we reorganized the Related Work section into two subsections: one for attacks and the other for defenses.
%
Each subsection is further divided into two paragraphs, the first discussing related studies and the second highlighting the differences between our work and other studies.
%
Minor topics within these subsections are now emphasized using \textit{italic} typeface for clarity.






% \end{auxmulticols}

